Diverse Imitation Learning via Self-Organizing Generative Models

Imitation learning is the task of replicating expert policy from demonstrations, without access to a reward function. This task becomes particularly challenging when the expert exhibits a mixture of behaviors. Prior work has introduced latent variables to model variations of the expert policy. However, our experiments show that the existing works do not exhibit appropriate imitation of individual modes. To tackle this problem, we adopt an encoder-free generative model for behavior cloning (BC) to accurately distinguish and imitate different modes. Then, we integrate it with GAIL to make the learning robust towards compounding errors at unseen states. We show that our method significantly outperforms the state of the art across multiple experiments.

==> backups.tex <==
% \textbf{Hoeffding's Theorem}\footnote{http://www.stat.cmu.edu/~larry/=sml/Concentration-of-Measure.pdf}. If $Z_1, Z_2, \ldots, Z_N$ are independent with \hbox{$\mathbb{P}(a_i \leq Z_i \leq b_i) = 1$}, having the same expected value $\mu=\mathbb{E}[Z_i]$, then for any $\epsilon > 0$,
% \begin{equation}
%     \mathbb{P}\left(\left|\bar{Z}_N-\mu\right|<\epsilon\right) \leq 2e^{-2N\epsilon^2/c}
% \end{equation}
% where $c=\frac{1}{N}\sum_{i=1}^N (b_i-a_i)^2$, $\bar{Z}_N=\frac{1}{N}\sum_{i=1}^N Z_i$.

% Considering eq \ref{eq:log-likelihood}, let us denote the following:
% \begin{subequations} \label{eq:hoeffding-notation}
% \begin{align}
%     &Z_i = \exp\left(-\frac{||f_\theta(\vz_i)-\vy||^2}{2\sigma^2}\right)\\
%     &\mu = \E_{\vz^{(i)}}[Z_i]=\E_\ensemble \left[ \bar{Z} \right]
% \end{align}
% \end{subequations}
% According to Hoeffding's theorem, given sufficient samples, with high probability we have:
% \begin{equation}
%     \displaystyle 
%     \left|\bar{Z}_N-\mu\right|<\epsilon
% \end{equation}
% Subtracting \ref{subeq:jensen} from \ref{subeq:montecarlo2} and plugging in the notations in eq \ref{eq:hoeffding-notation}, we obtain:
% \begin{subequations}
%     \begin{align}
%     \displaystyle 
%     \left|\log\mu-\E_\ensemble\log\bar{Z}_N\right|&\leq\\
%     \E_\ensemble\left|\log\mu-\log\bar{Z}_N\right|&\leq\\
%     \E_\ensemble\left|\log\mu - \log\left(\mu-\epsilon\right)\right|&= \label{subeq:concave-log}\\
%     \left|\log\mu - \log\left(\mu-\epsilon\right)\right|&< \delta
%     \end{align}
% \end{subequations}
% where \ref{subeq:concave-log} is due to concavity of logarithm. Derivation above shows that ``Jensen gap'' can be closed arbitrarily tightly with high probability. Moreover, for a finite $N$, the lower bound in \ref{subeq:boeltzmann} is also asymptotically tight as $\sigma^2\rightarrow 0$, since the summands of \ref{subeq:jensen} are essentially forming an unnormalized Boeltzmann (i.e. softmax) distribution.


% OUTLINE:
% 0. We want to bridge what SOG does -- maximizing the conditional likelihood at the optimal latent code -- with the optimization of the marginal likelihood
% 1. \cite{Chib (1995)} basic marginal likelihood identity: log-likelihood (\log p(y | x, theta)) = conditional log-likelihood - flexibility (\log(posterior / prior))
% 2. Assuming unit Gaussian prior and N(mu(x,y,theta), sigma(x,y,theta)) posterior, we have analytical form of the best latent code z* in terms of mu(x,y,theta) and sigma(x,y,theta), and therefore also the analytical form of the flexibility
% 3. We need to show that along the training of theta: \mu^T(1-\Sigma)^{-1}\mu + \log \det (\Sigma) decreases
%    a) $\mu(\theta)$ is bounded within a constant range
%    b) $\log\det(\Sigma)$ decreases to a properly small level


In this section we argue that \Cref{alg:sog} can be applied to the case where the latent code is a continuous variable with a unit Gaussian prior:
\begin{equation}
    p(\vz) = \normdis (\vz;\boldsymbol{0}, \mI)
\end{equation}
We first note that the following identity, known as marginal likelihood identity \citep{chib1995marginal}, holds for all latent code $\vz$ due to the Bayes' rule. 
\begin{equation} \label{eq:bayes}
    \underbrace{\log p(\vy | \vx; \boldsymbol\theta)}_\text{data log-likelihood} = \underbrace{\log p(\vy | \vz, \vx; \boldsymbol\theta)}_\text{SOG objective} - \underbrace{\log \frac{p(\vz | \vx,\vy;\boldsymbol\theta)}{p(\vz)}}_\text{gap}; \ \forall \vz.
\end{equation}
The left-hand side of \Cref{eq:bayes} is the log-likelihood of the data, and the first term on the right-hand side is the SOG objective function. Therefore, between the data log-likelihood, and the SOG term that is being optimized, there is a gap equal to the second term on the right-hand side.

To analyse this gap, we first realize that the log-likelihood is not a function of $\vz$, the optimal $\vz$ in \Cref{alg:sog} also maximizes the gap:
% $\max_{\theta} \log P(\vy \given \vz^*, \vx, \theta)$ leads to $\max_{\theta}P(\vy \given \vx, \theta)$\\
% $\log p(\vy \given \vx, \theta) = \log p(\vy \given \vz, \vx, \theta) - \log \frac{p(\vz \given \vy, \vx, \theta)}{p(\vz)}$
\begin{subequations}
\begin{align}
    \vz^* &= \argmax_{\vz} \log p(\vy | \vz, \vx; \boldsymbol\theta) \\ 
    &= \argmax_{\vz} \log \frac{p(\vz | \vx,\vy; \boldsymbol\theta)}{p(\vz)} \label{eq:argmax-gap}
\end{align}
\end{subequations}
We further assume that the function $f$ is implemented by a high capacity neural network, and as a result, the posterior can take an arbitrary form \citet{kingma2013auto}, e.g. a Gaussian: 
\begin{equation}
    p(\vz | \vy, \vx, \boldsymbol\theta) = \mathcal{N} (\vz;\boldsymbol\mu_{\boldsymbol\theta}(\vx, \vy), \boldsymbol\Sigma_{\boldsymbol\theta}(\vx, \vy)),
\end{equation}
Denoting $\boldsymbol\mu=\boldsymbol\mu_{\boldsymbol\theta}(\vx, \vy)$ and $\boldsymbol\Sigma=\boldsymbol\Sigma_{\boldsymbol\theta}(\vx, \vy)$ to avoid clutter, the optimal solution for \Cref{eq:argmax-gap} can be written as:
\begin{equation}
\begin{aligned} \label{eq:z-star}
    \vz^* &= \argmax_\vz -\frac{1}{2}\left[(\vz-\boldsymbol\mu)^T\boldsymbol{\Sigma}^{-1}(\vz-\boldsymbol\mu)^T\right]-\frac{1}{2}\log\det\boldsymbol\Sigma+\frac{1}{2}\vz^T\vz\\
    &=\begin{cases}
    (\mI-\boldsymbol\Sigma)^{-1}\boldsymbol\mu, & \text{if } \mI-\boldsymbol\Sigma \succ 0\\
    \text{unbounded},              
    & \text{otherwise}
    \end{cases}
\end{aligned}
\end{equation}
Note that since the network is trained to create mutual information between the data points and the unit variance latent code Normal distribution, we expect that the uncertainty in the posterior distribution should be less than in the prior distribution in all directions.  Thus the condition $(\mI-\boldsymbol\Sigma) \succ 0$ should hold. 
Plugging $\vz^*$ into (\ref{eq:argmax-gap}), and rewriting the covariance matrix in the diagonalized form, $\boldsymbol\Sigma=\mQ\boldsymbol\Lambda\mQ^T$ and $\boldsymbol\Sigma^{-1}=\mQ\boldsymbol\Lambda^{-1}\mQ^T$, we obtain:
\begin{subequations}
\begin{align}
    &\max_{\vz} \, \log \frac{p(\vz | \vx,\vy; \boldsymbol\theta)}{p(\vz)}\\
    &=-\frac{1}{2}\left[(\vz-\boldsymbol\mu)^T\boldsymbol{\Sigma}^{-1}(\vz-\boldsymbol\mu)^T\right]\:\Bigr|_{\vz=\vz^*} \; -\frac{1}{2}\log\det\boldsymbol\Sigma\\
    &=\frac{1}{2}\left[\vz^T(\mI-\boldsymbol\Sigma^{-1})\vz+2\boldsymbol\mu^T\boldsymbol\Sigma^{-1}\vz-\boldsymbol\mu^T\boldsymbol\Sigma^{-1}\boldsymbol\mu\right]\Bigr|_{\vz=\vz^*} \; -\frac{1}{2}\log\det\boldsymbol\Sigma\\
    &=\frac{1}{2}(\mQ^T\boldsymbol\mu)^T(\mI-\boldsymbol\Lambda)^{-1}(\mQ^T\boldsymbol\mu)-\frac{1}{2}\log\det\boldsymbol\Sigma\\
    &=\frac{1}{2}\boldsymbol\mu^T\left(\mQ(\mI-\boldsymbol\Lambda)\mQ^T\right)^{-1}\boldsymbol\mu-\frac{1}{2}\log\det\boldsymbol\Sigma\\
    &=\frac{1}{2}\boldsymbol\mu^T(\mI-\boldsymbol\Sigma)^{-1}\boldsymbol\mu-\frac{1}{2}\log\det\boldsymbol\Sigma \\
    &= g(\boldsymbol\mu, \boldsymbol\Sigma) \label{eq:gap}
    % &=-\frac{1}{2}\left[(\vz-\boldsymbol\mu)^T\boldsymbol{\Sigma}^{-1}(\vz-\boldsymbol\mu)^T\right]-\frac{1}{2}\log\det\boldsymbol\Sigma\:\Bigr|_{\vz=\vz^*}
\end{align}
\end{subequations}

We now argue that when the optimization in \Cref{alg:sog} reaches the optimum, one can make the following assumptions:
\begin{enumerate}
    \item Magnitude of $\boldsymbol\mu_\theta$ is bounded within a constant range; because the sampling scheme in \Cref{alg:sog} implies optimization of the loss function for values of $\vz$ that are samples of a unit Gaussian prior.

    \item One can easily show that $\boldsymbol\mu^T(\mI-\boldsymbol\Sigma)^{-1}\boldsymbol\mu=\Tr(\boldsymbol\mu \boldsymbol\mu^T (\mI-\boldsymbol\Sigma)^{-1}) \leq \|\boldsymbol\mu\|^2 \sqrt{\Tr((\mI-\boldsymbol\Sigma)^{-2})}.$ This uses the inequality that if $A$ and $B$ are positive semidefinite matrices, then $\Tr(AB) \leq \sqrt{\Tr(A^2)\Tr(B^2)}$.
    Now using the spectral decomposition of the covariance matrix, \[\boldsymbol\Sigma = Q \boldsymbol\Lambda Q^T, \quad \text{where $Q$ is orthogonal},\] we get $g(\boldsymbol\mu, \boldsymbol\Sigma) \leq \frac{1}{2}(c \sqrt{\Tr((I- \boldsymbol\Lambda)^{-2})}-\log\det\boldsymbol\Lambda)= h(\boldsymbol\Lambda)$. Recall that $\boldsymbol\Lambda \leq \mI$ and with training the elements of $\boldsymbol\Lambda$ decrease as the posterior gets sharper. Then one can show that $h(\boldsymbol\Lambda)$ decreases initially with training when the the elements of $\boldsymbol\Lambda$ are not too small. Thus, going back to \Cref{eq:bayes} we get that  (data log-likelihood) $\geq$ -(SOG-loss + $h(\boldsymbol\Lambda)$) and with iterations both terms in this lower bound increases initially until the eigenvalues become too small. Thus the log-likelihood of the  data is increased as training progreses. 
    
    \item Next, assuming no overfitting of the data by the network $f$ (this is possible even with a network with high expressive power), one is guaranteed that  
    % , and the reconstruction error of data samples does not become very small.
    the entries of $\boldsymbol\Sigma$ are not too small even at convergence, so that $\log\det(\boldsymbol\Sigma)$ is bounded and $g(\boldsymbol\mu, \boldsymbol\Sigma)$ stays bounded. In particular, at convergence the parameters, $\theta$ are not too far from the point that maximizes the data log-likelihood.%, because as the training continues, different regions of the latent space become organized towards producing different modes of the data.
\end{enumerate}
Given the assumptions above of Gaussian posterior, we have shown that the 
%gap calculated in \Cref{eq:gap} is not only bounded but it decreases initially in the training process, and therefore the optimization objective in 
\Cref{alg:sog} maximizes the data log-likelihood and by avoiding overfitting it stays close to the maximum point.

% $\vz^*= (\mI - \Sigma)^{-1}\mu$, 
% $\log \frac{p(\vz^* \given \vx, \vy, \theta)}{p(\vz^*)} = \frac{1}{2} [\mu^T(\mI - \Sigma)^{-1}]\mu - \log det(\Sigma)$

-----

\textbf{Alternative Algorithms}
% The objective function in \Cref{eq:max-likelihood} joins the optimization of the parametric model (solving for $\bm\theta$) with the latent space optimization (solving for $\mZ$). SOG addresses it with straightforward randomized search over latent space.

Typically, maximum likelihood problems involving latent variables are solved with expectation-maximization (EM) algorithms or variational inference methods such as variational autoencoder (VAE). These methods try to find a $\theta$ that maximizes the marginal likelihood as shown in \Cref{eq:max-marginal-likelihood}, while calculating or estimating the posterior distribution of the latent codes. The $\mZ$ can then be found with maximum \textit{a posteriori} (MAP) estimator.

Although EM or variational inference methods can be used to solve \Cref{eq:max-likelihood}, the difference between \Cref{eq:max-likelihood} and their marginalized objective \Cref{eq:max-marginal-likelihood} has several implications.

Points can be made: 1. not marginalizing the latent variables encourages faster mode separation; 2. not marginalizing the latent variables lead to lower data-fitting error -- can be seen as the effect of having additional parameters; 3. not marginalizing the latent variables can be safe from over-fitting because of the SOG effect
% see \Cref{appx:continuous,appx:em} for detailed discussion.

From another perspective, EM and VAE can be bridged with SOG by algorithmic changes. For example, one can modify the latent code search mechanism in SOG (\Cref{alg:sog}) and search for latent codes $\vz^{(i+1)}_j$ locally around the previously selected latent code $\vz^{(i)}_j$ of each data point. The $\{\vz^{(i)}_j\}$'s can be seen as non-parametric point estimations of the latent posterior. Further, if a parametrized model is used for the proposal of such local search regions, the algorithm essentially becomes variational autoencoder (VAE).

% Soft assignment of data points to the discrete latent codes can also be introduced as one possible regularization.%, so that the update of $\bm \theta$ is not
%  In the case of discrete latent codes where exhaustive search of latent codes is tractable,

% As we can see from SOG algorithm, 
% \begin{subequations}

% \end{subequations}

-----

==> results/performance-vs-lambda.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
    \begin{center}
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \adjincludegraphics[width=\textwidth,trim={{.05\width} {.05\height} {.05\width} {.1\height}},clip]{fig/robustness/unperturbed}
        \caption{Unperturbed policy}
    \end{subfigure}
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \adjincludegraphics[width=\textwidth,trim={{.05\width} {.05\height} {.05\width} {.1\height}},clip]{fig/robustness/perturbed}
        \caption{Perturbed policy}
    \end{subfigure}
    \caption{Performance of \Cref{alg:sog-gail} for different choices of $\lambda_S$, under unperturbed and perturbed conditions.}
    \end{center}
\end{wrapfigure}

==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section \textbf{\{REMOVED\}}}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerNA{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{In section \ref{sec:background} we thoroughly set assumptions.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{In section \ref{sec:sog-imitation}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Full code along with instructions are included as supplementary material, and we will link to our \texttt{github} repository after the double blind review phase.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The training details are included as supplementary material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We tried to thoroughly cite code bases and papers used.}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> sections/method.tex <==
\section{Method} \label{sec:method}

In this section, we aim to propose an algorithm for imitation of diverse behaviors. We first introduce a generative model for learning the distribution of arbitrary datasets. Namely, let $\vx$ and $\vy$ respectively denote an input data point and a corresponding output data point. We assume that $\vy$ is generated through a two-stage random process:
\begin{enumerate}
\item A  latent variable $\vz$, independent of $\vx$, is sampled from a prior distribution $p(\vz)$. This prior can be a given discrete distribution over $K$ categories with probability masses $\pi_1,\ldots,\pi_K$, or an arbitrary continuous distribution, e.g. a multivariate Gaussian $\displaystyle p(\vz)= \mathcal{N} ( \vz ; \mathbf{0}, \mI)$.
\item A value $\vy$ is sampled from a conditional distribution $p(\vy|\vz, \vx;f)$  of the following form:
\begin{equation} \label{eq:posterior}
    p(\vy|\vz,\vx;f) = \mathcal{N} ( \vy ; f(\vz,\vx), \sigma^2\mI),
\end{equation}
where $f$ maps $\vz$ and $\vx$ to the mean of the distribution, and $\sigma^2$ is the isotropic noise variance in the space of $\vy$.
\end{enumerate}

\subsection{The Self-Organizing Generative Model} \label{sec:general-sog}
Suppose that a dataset $\mathcal{D}=\{(\vx_{i},\vy_{i})\}_{i=1}^N$ consists of $N$ i.i.d samples generated by the process above. To learn the generative process underlying the dataset, one needs to restrict the estimation of function $f$ within a family of parameterized functions, e.g. neural networks $f_{\boldsymbol\theta}$ with weight parameters $\boldsymbol\theta$. 
% We design an algorithm  to estimate $\boldsymbol\theta$, such that the samples generated by the inferred model match the distribution of the dataset.
% , where the corresponding latent variable samples $\{\vz_{i}\}$ are kept hidden and the function $f(\cdot)$ is unknown. 
We propose learning the parameters $\boldsymbol\theta$ by randomly initializing them, followed by a two-step iterative procedure:
\begin{enumerate*}[(1)]
\item given current $\boldsymbol\theta$, for each data point, we estimate the latent variable $\vz^* = \argmax_{\vz} p(\vy|\vz,\vx;\,\boldsymbol\theta)$ \item given the estimated $\vz^*$, we take a gradient step on $\boldsymbol\theta$ to increase the likelihood $p(\vy|\vz^*,\vx;\,\boldsymbol\theta)$.
\end{enumerate*} We note that both steps increase $p(\vy|\vz,\vx;\,\boldsymbol\theta)$, guaranteeing convergence. The resulting method is presented in \Cref{alg:sog}.

% \iffalse We discuss the naming of the algorithm in \Cref{sec:sog-properties}.


% \textcolor{gray}{One set of
% models can be derived by maximizing the log-likelihood of the observed data, over both the shared parameters $\boldsymbol\theta$, and an assignment $\vz_i \in \{1,\ldots, K\}$ for each data point $(\vx_{i},\vy_{i})$:}
% % \begin{subequations}
% \begin{align}\label{eq:max-likelihood}
% \begin{split}
%     &\max_{\substack{\boldsymbol\theta,\mZ}}\sum_{i=1}^N\log p(\vy_{i}|\vz_i,\vx_{i};\,\boldsymbol\theta), 
%     \\&\text{where } \mZ=\{\vz_1, \ldots, \vz_N\} \quad \text{and} \quad \vz_i \in \{1,\ldots, K\}.
% \end{split}
% \end{align}
% % \end{subequations}

% The rest of this section is organized as follows. In \Cref{sec:general-sog}, we introduce an algorithm named Self-Organizing Generative Model (SOG) to \textcolor{gray}{efficiently solve the optimization problem of \Cref{eq:max-likelihood}}. In \Cref{sec:sog-imitation}, we adopt this algorithm for multimodal imitation learning in BC and GAIL settings.
% In \Cref{sec:sog-analysis}, we briefly mention the \textcolor{blue}{relationship} between optimization of \Cref{eq:max-likelihood} (as adopted by SOG), and the principle of maximum likelihood estimation, where the data likelihood is marginalized over the latent variable. We expand this relationship in the appendix due to space limits. % That is, instead of computing a single optimal assignment of $\vz_i$ (as in the case of the above optimization), a distribution $p(\vz_i=k| \text{\texttt{data}};\,\boldsymbol\theta);\,k=1,\ldots, K$ is computed. This connection is expanded later in \Cref{appx:em,appx:continuous} due to space limits.  
% Finally, in \Cref{sec:sog-properties}, we elaborate on some additional aspects of the SOG model.
% %\subsection{The SOG Algorithm in General} \label{sec:general-sog}
% In \Cref{alg:sog}, we \textcolor{blue}{propose a method} to optimize \Cref{eq:max-likelihood} in both cases of discrete and continuous latent variables.
% \fi

\begin{algorithm}[H]
	\caption{Self-Organizing Generative Model (SOG)}
	\label{alg:sog}
	\begin{algorithmic}[1]
	    \State \textbf{Define}: Loss function $\mathcal{L}\left(\hat{\vy},\vy\right)\coloneqq ||\hat{\vy}-\vy||^2$
	    \State \textbf{Input:} Initial parameters of policy network $\boldsymbol\theta_0$
		\For {$epoch=1,2,\ldots$}
		     \For {$iteration=1,2,\ldots$}
		        \parState{Sample a minibatch of $N_\text{data}$ data points $ (\vx_i,\vy_i)$ from the dataset.}
		        \For {$i=1,2,\ldots,N_\text{data}$}
    		        \State Sample $N_z$ latent codes $ \vz_j \sim p(\vz)$. \label{alg:sog:latent-batch}
    		      %  \State Calculate all candidate generated samples $\displaystyle f_\theta(\vz^{k)})$.
    	           \State Calculate $\vz_i\coloneqq\arg\min_{\vz_j}\mathcal{L}\left(f_{\boldsymbol\theta}(\vz_j,\vx_i), \vy_i\right)$. \label{alg:sog-best-z}
    	       \EndFor
    	       \parState{Calculate $ \mathcal{L}_{\mathrm{SOG}}=\sum_{i=1}^{N_\text{data}}\mathcal{L}\left(f_{\boldsymbol\theta}(\vz_i,\vx_i), \vy_i\right)$ and its gradients w.r.t. ${\boldsymbol\theta}$.} \label{alg:sog-loss}
    	       \parState{Update $f_{\boldsymbol\theta}$ by stochastic gradient descent on ${\boldsymbol\theta}$ to minimize $\mathcal L_{\mathrm{SOG}}$.}
		    \EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}
In this algorithm, if the latent variable is discrete, $\vz^*$ is exhaustively searched over $\vz\in\{1,\ldots,K\}$. In the continuous case, $\vz^*$ is searched over samples of the prior $p(\vz)$. 

A closely related approach for model optimization is maximizing the marginal likelihood $p(\vy|\vx;\,\boldsymbol\theta)$ with respect to $\boldsymbol\theta$. In the framework of Expectation Maximization (EM) \citep{bishop2006pattern}, this can be achieved by iterating between:
\begin{enumerate*}[(1)]
    \item calculating the posterior $p(\vz|\vy,\vx;\,\boldsymbol\theta)$ for the current $\boldsymbol\theta$
    \item updating the model parameters $\boldsymbol\theta$ to increase the likelihood of data, marginalized over the posterior of step 1.
\end{enumerate*}
The SOG algorithm replaces step 1 with computing a maximum likelihood [point] estimate for $\vz$. The relationship and equivalence between \Cref{alg:sog} and optimization of the marginal likelihood are included in \Cref{appx:em,appx:continuous}.

\iffalse
In a marginal likelihood framework, a posterior distribution for $\vz_i$ is estimated. In our SOG algorithm, we instead obtain a point estimate $\vz_i = \vz_i^*$.  Formal relationships and equivalences between the SOG algorithm --that iteratively computes an MLE of $\vz$ for given $\boldsymbol\theta$ and then increases the likelihood of data computed at these estimates of $\vz$ by updating the model parameters $\boldsymbol\theta$ -- and algorithms based on maximizing the marginalized likelihood -- that iteratively computes a posterior distribution of $\vz$ for given $\boldsymbol\theta$, and then increases the likelihood of data marginalized over the distribution of $\vz$ by updating the model parameters $\boldsymbol\theta$ -- are included in \Cref{appx:em,appx:continuous}.
\fi
% \iffalse
% In \cref{alg:sog-bc:latent-batch} of the algorithm, if the latent variable is discrete, an exhaustive search is performed over $\vz\in\{1,\ldots,K\}$. In the continuous case, the optimal $\vz$ is searched over samples of the prior distribution $p(\vz)$. 

% This algorithm performs a two-step optimization over each batch of data:
% \begin{enumerate*}[(1)]
% \item given current $\boldsymbol\theta$, finding the best latent codes; \item given the best latent codes, taking a gradient step on $\boldsymbol\theta$.
% \end{enumerate*}
% Both steps decrease the same loss function, guaranteeing convergence. We discuss the naming of the algorithm in \Cref{sec:sog-properties}.
% \fi
\subsection{Adopting SOG for Multimodal Imitation Learning}
\label{sec:sog-imitation}
% \vspace*{-2ex}
In the following, we introduce two approaches for multimodal imitation learning: 
\begin{enumerate*}[(1)]
    \item adopting SOG for multimodal BC, and
    \item combining multimodal BC with GAIL using SOG.
\end{enumerate*}
Due to space limits, the corresponding algorithms are presented in \Cref{appx:algorithms}.
\subsubsection*{Multimodal Behavior Cloning with SOG} We adopt \Cref{alg:sog} for learning the relationship between state-action pairs in a multimodal BC setting. We enforce an additional constraint that the latent code is shared across each trajectory. Hence, we propose \Cref{alg:sog-bc}.
\subsubsection*{Multimodal Combination of BC and GAIL using SOG}
Next, we introduce \Cref{alg:sog-gail}, where we combine SOG, as a means for BC, with GAIL to ensure robustness towards unseen states. This algorithm is inspired by \citet{jena2020augmenting}, which in a unimodal setting optimizes a weighted sum of BC loss and the GAIL ``surrogate'' loss (see \Cref{appx:gail-optim}).
% \vspace*{-2ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                   BEGIN BACKUP                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{\label{sec:sog-analysis}Analysis of SOG}
We establish the connection between \Cref{alg:sog} and maximum likelihood estimation in \Cref{appx:em,appx:continuous}. In this section, we present a summary of the analysis.
\subsubsection{Discrete Latent Variable}\label{sec:hard-assignment} 
% \vspace*{-2ex}

Expectation-maximization (EM) is a general technique for finding maximum likelihood estimators in  models involving latent variables \citep{dempster1977maximum}. We can apply EM to the maximum likelihood \textbf{problem of \Cref{eq:max-likelihood}}, and obtain an iterative procedure alternating between two steps:
\begin{enumerate}
    \item \textbf{Expectation Step.} At iteration $t$, calculate the posterior probabilities,
    \begin{equation} \label{eq:em-e}
        r_{ik}^t= p(\vz_i=k\, |\, \vx_i,\vy_i;\, {\boldsymbol\theta}^{t},\{\pi_j^{t}\}_{j=1}^K).
    \end{equation}
    \item \textbf{Maximization Step.} Update $\boldsymbol\theta^{(t+1)}$ and the prior probabilities $\{\pi_j^{(t+1)}\}_{j= 1}^K$ by maximizing the expectation value,
    \begin{equation} \label{eq:em-m}
        \sum_{i=1}^N r_{ik}^t \sum_{k=1}^K \log p(\vy_i,\vz_i=k \:|\:\vx_i, \boldsymbol\theta,\{\pi_j\}_{j=1}^K).
    \end{equation}
\end{enumerate} 

In \Cref{appx:em}, through a toy numerical experiment, we verify that EM converges to local optima of the maximum likelihood objective. However, we observe that the speed of convergence is relatively slow. 
% Besides, in general EM requires storing $\gamma_{ik}$'s, leading to a storage cost that grows linearly in the number of data points. 
On the other hand, our toy experiment suggests that the posterior probabilities  $r_{ik}^t$  asymptotically converge to one-hot assignments \textbf{(under which property of data?)}. That is,  if $t$ is large enough, then $r_{ik}^t \rightarrow \gamma_{ik} \in \{0, 1\}$, where for all $i$, there exists a value $j$ such that $\gamma_{ij} = 1$ and $\gamma_{ik} = 0; \forall k\neq j$. This implies that at convergence, each data point pair $(\vx_{i},\vy_{i})$ is assigned a unique latent code $\vz_{i} = j$. 

% analysis in \Cref{appx:em} supporting the convergence of posterior probabilities to such binary extremes

Observations above motivate us to directly search over one-hot posterior probabilities. \textbf{This hard assignment method }leads to combinatorial optimization problem  for optimizing the model parameters:
\begin{equation}
\label{eq:gen-cluster}
\begin{aligned}
    \min_{{\gamma}_{ik}} \min_{\boldsymbol\theta} \sum_{k=1}^K \sum_{i=1}^N \gamma_{ik} \norm{f(\vz_{i}=k,\vx_{i};{\boldsymbol\theta}) -\vy_{i}}^2,
\end{aligned}
\end{equation}
where $\gamma_{ik}$ is the binary indicator variable as defined above, and the $L_2$ error follows from the log probabilities in \Cref{eq:em-m}. 
% We shall consider a hard version of the EM algorithm to solve the optimization problem (\ref{eq:gen-cluster}): 
% \begin{enumerate}[(i)]
%     \item For a fixed $\boldsymbol\theta$ greedily pick the best latent code that leads to the least fitting error for each data point. For each data point $i$, this is equivalent to determining the latent code, say $j$,  with  maximum posterior probability, $r_{ij}$, to $1$ and setting the rest of $r_{il}=0$;
%     \item Optimize the model parameter $\boldsymbol\theta$ with the corresponding latent code assignments. \iffalse This step makes the additional assumption that the prior is uniform:  $\pi_j=\frac{1}{K}$. \fi
% \end{enumerate}
\textbf{This hard assignment method} is closely analogous to the derivation of the $K$-means algorithm from a corresponding soft EM in Gaussian mixture models \citep{pml1Book}.
Our toy experiment in \Cref{appx:em} illustrates that \textbf{hard-em} leads to faster convergence, and achieves \textbf{better} local maxima. 







% \vspace*{-2ex}

\subsubsection{Continuous Latent Variable} \label{sec:continuous}
% \vspace*{-1.5ex}
%\textbf{and the relationship with other non-adversarial generative models.} 
%For the continuous latent variable case, we follow a similar framework as  in the discrete case: (i) For a fixed $\boldsymbol\theta$ search among the samples of continuous latent space for the best code $\vz_i^*$ that leads to the least fitting error for each data point $(\vx_i,\vy_i)$; (ii) Optimize for $\boldsymbol\theta$ by training the model for output $\vy_i$, and input $(\vx_i,\vz_i^*)$.  

% The analysis for the continuous case is given in \Cref{appx:continuous}. Herein, we summarize some of the key characteristics of the continuous case and the resulting SOG algorithm:
% \textbf{Relationship with other non-adversarial generative models.} 
% ? resembles VAE 
% ... Unlike conventional non-adversarial generative models such as the VAE, the SOG model does not require an encoder.  In VAE, the encoder is used to learn a  posterior distribution $p(\vz| \vx_i,\vy_i;\, \theta)$, whose samples are used to 
\textbf{VAEs train the decoder...} In contrast, \Cref{alg:sog} trains the decoder by searching for a latent code $\vz$ that maximizes the likelihood $p(\vy | \vx, \vz ;\: \boldsymbol\theta)$. In \Cref{appx:continuous}, we show that this is equivalent to maximizing the ratio of the posterior to the prior, $\dfrac{p(\vz|\vx_i,\vy_i;\: \boldsymbol\theta)}{p(\vz)}$. %
% relate the $\max$ operation in SOG to the posterior distribution of the data points and
Accordingly, we show that under mild assumptions, the continuous version of the SOG also leads to the maximization of the marginal log-likelihood of the data $p(\mY | \mX;\: \boldsymbol\theta)$. 
%Related ``encoder-free'' frameworks have been recently considered for image synthesis \citep{bojanowski2017optimizing,hoshen2019non}.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    END BACKUP                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{\label{sec:sog-analysis}Analysis of SOG} % TODO: maybe this section should be put before the algorithm listings
% ----
% \textbf{Arash's suggestion for this section.}
% \textcolor{gray}{\Cref{alg:sog} optimizes the non-marginalized likelihood of \Cref{eq:max-likelihood}. However, it can be shown that this algorithm is also related to optimizing the marginalized likelihood of the data, i.e.:
% \begin{equation}
% \label{eq:max-marginal-likelihood}
% \max_{\boldsymbol\theta}\sum_{i=1}^N \log \int p(\vy_i|\vz, \vx_i; \, \boldsymbol\theta)p(\vz)d\vz.
% \end{equation}
% We characterize the relationship between \Cref{alg:sog} and \Cref{eq:max-marginal-likelihood} in the appendix due to space limits. We analyse discrete and continuous latent variables separately in  \Cref{appx:em,appx:continuous}.}
\iffalse
\blue{As shown in \Cref{eq:max-likelihood}, SOG assumes the log-likelihood conditioned on $\mZ$ as the maximization objective, where the latent variables 
%TIANYI's suggestions commented below
\iffalse(or so-called latent codes, as they encode the modality information)\fi $\mZ$ are included as optimization variables in addition to $\vtheta$.}
% >>> explained already below algo 1
% Concretely, SOG repeats the following two steps:
% \begin{enumerate}[(1)]
%     \item Select the best value of the latent variable $\mZ$ among a set of candidates
%     \item Update the model parameters $\vtheta$ to increase likelihood with $\mZ$ being the selected value from (1).
% \end{enumerate}

% As shown in \cref{alg:sog}, the algorithm optimizes the objective by alternatingly optimizing for $\mZ$ and for $\vtheta$.

\blue{Including $\mZ$ as an optimization variables in addition to the neural model parameters leads to the concern: could these extra optimization variable cause ungeneralizable memorization and overfitting? In other words, during the training.}
% In contrast, the marginal likelihood where latent variables are marginalized is believed to 
% The first step is attended differently for the case where $\vz$ is discrete and where $\vz$ is continuous.

% See appendix C for more discussions relating to marginalized likelihood
\newcommand{\flexibility}{\textsf{flexibility}}
\blue{
\begin{enumerate}
\item SOG's loss is non-marginalized, and essentially introduces more parameters, although the model complexity is not changed. The concern is that this could lead to overfitting
\item The overfitting effect is quantified with ``\flexibility{}'' (\cite{rougierExactFormOckham2020}), \(\log \frac{p(\vz \given \vx, \vy; \vtheta)}{p(\vz)}\). Intuitively, if the model is able to concentrate its posterior probability into a small region in the latent space, the \flexibility{} is high.
\begin{enumerate}
\item In fact, the \flexibility{} bridges the non-marginalized likelihood and the marginalized likelihood through the basic marginal likelihood identity (\cref{eq:BMI})
\item The \flexibility{} in the discrete case is bounded above by \(\log K\)
\begin{enumerate}
\item Therefore SOG should behave similarly as EM, especially when assuming the data has well-separated modes
\item Our toy example verifies this
\end{enumerate}
\item The \flexibility{} in the continuous case is more concerning compared to the discrete case. Continuous code can theoretically encode infinite information, so a model could have take advantage of the latent space to make ungeneralizable memorization.
\begin{enumerate}
\item VAE tackles this by considering the \flexibility{}. It uses the marginalized likelihood as its objective, and algorithmically it adds finite amount of random perturbation to the MAP of the latent code during training.
\item SOG, on the other hand, also has random perturbation added to the MAP, due to the randomized search.
\item Even if there is no explicit regularization, autoencoders in practice don't make too much memorization. This is because of the continuity of NN models.
\end{enumerate}
\end{enumerate}
\end{enumerate}
}

\blue{REMINDER: must make references to \Cref{appx:em,appx:continuous}}
\fi
\subsection{Further Properties of SOG} \label{sec:sog-properties}
\subsubsection*{Sample Complexity} Training procedure of \Cref{alg:sog}, given a high-dimensional continuous latent variable, requires a prohibitively large number of latent code samples (\cref{alg:sog:latent-batch} of the algorithm). In \Cref{appx:extended-sog}, we propose a computationally efficient extension of this algorithm suited for high dimensions of the latent space.

\subsubsection*{Self-Organization in the Latent Space} In \Cref{appx:lipschitz-bounds}, we show that latent codes corresponding to nearby data points get organized close to each other. In addition, visual results in  \Cref{fig:fetch-latent} and \Cref{appx:extended-sog} show that different regions of the latent space organize towards generating different modes of data. Hence, the phrase ``self-organization'' in naming of \Cref{alg:sog} is justified.
% \textbf{IMAGE DATA}

%in Further, under the assumption of a uniform prior $p(\vz)$, and by employing the strategy of hard assignment (as used in the derivation of the $K$-means algorithm\citep{pml1Book}) the EM algorithm simplifies to a  case that corresponds to the following objective:
%MLE problem as the following discrete optimization problem, recognizing that the log of the assumed Gaussian likelihood is directly translated to $\normltwo$ norm:
%\begin{equation}
%\label{eq:gen-cluster}
%\begin{aligned}
 %   \min_{{l}_{ik}} \min_\theta %\sum_{k=1}^K \sum_{i=1}^N %l_{ik} \norm{f(\vz_{i}=k,\vx_{%i};\theta) -\vy_{i}}^2,
%\end{aligned}
%\end{equation}
%where $l_{ik} \in \{0, 1\}$ is a binary indicator variable, and for any $i$ there exists one and only one $j$ such that $l_{ij} = 1$ while $l_{ik} = 0$ for $k\neq j$. This implies that the data point pair $(\vx_{i},\vy_{i})$ is assigned the latent code $\vz_{i} = j$ %
%(equivalently, $\vz_{i} = e_j$, the corresponding one-hot code)
%and the function  $f_\theta(\vz_{i}=j,\vx_{i})$ is used to estimate $\vy_{i}$. 

%Let $\mathcal{C}_k = \{i \given l_{ik} = 1\}$ be the set of all data point indices that are assigned to the latent code $k$. Then solving the optimization problem in \cref{eq:gen-cluster} corresponds to determining an optimal clustering of the data points into $K$ sets, $\{\mathcal{C}_{1}, \cdots, \mathcal{C}_K\}$, such that the log-likelihood of the data is maximized by the respective generators $f_{\theta}^{(k)}(\cdot) \equiv f_\theta(\vz_{i}=k, \cdot)$, for $k=1, \cdots, K$.
% One pair of data, $(\vx_{i}, \vy_{i})$, defines a single-point mapping function $m_i: m_i(\vx_{i}) = \vy_{i}$. % This functional view of the data-label pairs is illuminating. It helps to recognize that a distance metric among the mapping functions (including $f^{(k)}_\theta$) can be induced from a metric in the data (label?) space
%Therefore \cref{eq:gen-cluster} can be re-written as
%\begin{align}
%\label{eq:cluster-opt}
 %   &\min_{\{\mathcal{C}_1,\cdo%ts,\mathcal{C}_K\}} \; %\sum_{k=1}^K \;\; %\left(\min_{f^{(k)}} \; %\sum_{(\vx, \vy) \in %\mathcal{C}_k} \norm{\vy - %f^{(k)}(\vx)} \right)
    % \\ =& %\min_{\{\mathcal{C}_1,\cdot%s,\mathcal{C}_K\}} \; %\sum_{k=1}^K \;\; \left( %\min_\theta \; \sum_{i \in %\mathcal{C}_k} \xi(f^{(k)}, %(\vx_i, \vy_i)) \right)
%\end{align}

%Again we compare \cref{eq:cluster-opt} with the objective of $K$-means clustering algorithm in \cref{prob:kmeans} to emphasize their similarity. This reveals that the case of discrete latent codes can be viewed as a generative clustering problem, where one jointly optimizes for both cluster assignments of data points and  the functions $\{f^{(k)}\}_{k=1}^K$ to fit the data points within each cluster.

%\begin{align}
%\label{prob:kmeans}
%    \min_{\{\mathcal{C}_1,\cdot%s,\mathcal{C}_K\}} \; %\sum_{k=1}^K \;\; %\left(\min_{\mu_k} \; %\sum_{\vx_{i} \in %\mathcal{C}_k} \norm{\vx_{i} - %\mu_k} \right)
    % = \min_{\{\mathcal{C}_1,\c%dots,\mathcal{C}_K\}} \; %\sum_{k=1}^K \;\; \left( %\min_{\{\mu_1,\cdots,\mu_K\%}} \; \sum_{\vx_{i} \in %\mathcal{C}_k} %\xi{(\vx_{i}, \mu_k)} %\right)
%\end{align}

%Note that the $f^{(k)}$ in \cref{eq:cluster-opt} are assumed to share the parameter $\theta$ and differ only due to the fed-in latent codes. This assumed form of $f^{(k)}$ can be considered as a regularization that prevents the learning of multiple completely disjoint models (one for each latent code assignment $\vz=k$) and in practice boosts the training process, because $\theta$ receives feedback from all data points regardless of the modality.

% This analogy to $K$-means is important because we can take $K$-means' approach to address this problem, which is the EM algorithm or its hard-assignment version. We show in the appendix that algo that solves this problems can be derived from the EM framework, and $K$-means' approach leads to SOG.

% Thus, the case of discrete latent codes can be viewed as a Generative Functional Clustering Problem (GFCP), where one jointly optimizes for both cluster assignments of data points and  the parameters $\theta$ that construct the functions $f_\theta(\cdot, \cdot)$.

% If $f_\theta(\cdot, \cdot)$ is realized using a DNN with a large enough number of parameters then one can achieve a small enough reconstruction error for almost any clustering of the input data. These clusters, however, need not correspond to the naturally occurring distinct modes present in  expert demonstrations: in principle, a DNN can learn any function, however non-smooth, given enough parameters, training data and computing power.

%The problem in \cref{eq:gen-cluster} (or \cref{eq:cluster-opt}) is a combinatorial optimization problem and a number of algorithms can potentially be used to find good minima. There are, however, several challenges of which perhaps the most important one relates to the approximation capabilities of DNNs. If $f_\theta(\cdot, \cdot)$ is realized using a DNN with a large enough number of parameters then one can achieve a small enough reconstruction error for almost any clustering of the input data. These clusters, however, need not correspond to the naturally occurring distinct modes present in  expert demonstrations: in principle, a DNN can learn any function, however non-smooth, given enough parameters, training data and computing power. To avoid such complex mapping in the decoder, we adopt the iterative framework of expectation-maximization (EM). The underlying goal is to perform least squares regression between $\vx$, $\vy$ pairs (conditioned on the one-hot latent codes) in incremental steps, while ensuring smoothness of the function $f_\theta$ w.r.t. its arguments. As shown in \Cref{lipschitz-bounds} our iterative EM framework ensures that data pairs $(\vx,\vy)$ that are close to each other, and hence, could be considered as belonging to the same mode, are mapped to the same latent variable $\vz$. Thus, data points that are close to each other  use the same mapping $f_\theta(\vz,\cdot)$, keeping it smooth and less complex.

%The connection between the case of discrete latent code and the $K$-means algorithm motivates the following iterative  optimization paradigm that we have termed as the SOG:
%\begin{enumerate*}[(a)]
 %   \item For a fixed $\theta$ greedily pick the best latent code that leads to the least fitting error for each data point;
 %   \item Optimize the model parameter $\theta$ assuming the picked latent code. Repeat.
%\end{enumerate*}





% The likelihood of an individual datapoint $\vy$ can be written as:
% \begin{subequations} \label{eq:likelhood}
%     \begin{align}
%     \displaystyle 
%     p_\theta(\vy)   & = \E_{\vz\sim p(\vz)} \left[ p_\theta(\vy | \vz)\right] \label{subeq:likelihood} \\
%                     & = \E_\ensemble \left[\frac{1}{N_z}\sum_{i=1}^{N_z} p_\theta(\vy | \vz_{i})\right], \hspace{0.45in} \vz^{(1)},\ldots, \vz^{(N_z)} \stackrel{\mathrm{i.i.d}}{\sim} p(\vz) \label{subeq:montecarlo1}
%     \end{align}
% \end{subequations}
% where in \ref{subeq:montecarlo1} the variable under expectation is replaced with its empirical mean. Taking the logarithm of both sides we obtain:
% \begin{subequations} \label{eq:log-likelihood}
%     \begin{align}
%     \displaystyle 
%     \log p_\theta(\vy) & = \log\E_\ensemble \left[\frac{1}{N_z}\sum_{i=1}^{N_z} p_\theta(\vy | \vz_{i})\right] \\
%         & = \log\E_\ensemble \left[C \sum_{i=1}^{N_z}  \frac{1}{N_z}\exp\left(-\frac{||f_\theta(\vz_{i})-\vy||^2}{2\sigma^2}\right)\right] \label{subeq:montecarlo2} \\
%         & \geq \E_\ensemble \left[ \log \left( C \sum_{i=1}^{N_z} \frac{1}{N_z}\exp\left(-\frac{||f_\theta(\vz_{i})-\vy||^2}{2\sigma^2}\right) \right)\right] \label{subeq:jensen}  \\
%         & \geq \E_\ensemble \left[\log \left( C\max_{i} \left\{ \frac{1}{N_z} \exp\left(-\frac{||f_\theta(\vz_{i})-\vy||^2}{2\sigma^2}\right)\right\}\right)\right] \label{subeq:boeltzmann} \\
%         & = C' -\frac{1}{2\sigma^2} \E_\ensemble \left[ \min_{i}||f_\theta(\vz_{i})-\vy||^2\right]. \label{subeq:simplified-min}
%     \end{align}
% \end{subequations}
% Equation \ref{subeq:montecarlo2} is the density of the Gaussian distribution in equation \ref{eq:posterior}, with constants $C$ (and $C'$) defined as appropriate. Inequality \ref{subeq:jensen} follows from Jensen's inequality, and is shown in Appendix \ref{appx:proof} to provide a tight bound for large enough $N_z$. Moreover, (\ref{subeq:boeltzmann}) is obtained by keeping only the largest summand. This bound also gets tighter as $\sigma$ decreases. As apparent from (\ref{subeq:simplified-min}), $\sigma$ only plays a role in scaling the magnitude of the gradient. 

% We optimize the lower bound of the maximum likelihood objective, by taking gradient of (\ref{subeq:simplified-min}). We also approximate the expectation in (\ref{subeq:simplified-min}) with one sample. Altogether, we first draw $N$ i.i.d samples $\displaystyle \vz_{i}$, then up to a constant factor the gradient of the log-likelihood can be written as:
% \begin{equation}
%     \displaystyle 
%     \nabla_\theta \log p_\theta(\vy)  \approx -\nabla_\theta \min_i
%     ||f_\theta(\vz_{i})-\vy||^2
% \end{equation}
% \vspace*{-2ex}


==> sections/method0.tex <==
\section{Method} \label{sec:method}

To enable imitation learning from diverse trajectories, we first introduce a novel generative model capable of learning arbitrary distributions.  For an input data point $\vx \in \mathbb{R}^n$, we assume that a corresponding output data point $\vy \in \mathbb{R}^m$ is generated by a two-stage random process:
\begin{enumerate}
\item A  latent variable $\vz$ (independent of $\vx$) is sampled from some prior distribution $p(\vz)$. The prior $p(\vz)$ can be a given discrete distribution over $K$ categories with probability masses $\pi_1\ldots\pi_K$, or a continuous variable in $\mathbb{R}^d$ with an arbitrary density, e.g. $\displaystyle p(\vz)= \mathcal{N} ( \vz ; \mathbf{0}, \mI)$.
\item A value $\vy$ is drawn from a conditional distribution $p(\vy|\vz, \vx;f)$  of the following form:
\begin{equation} \label{eq:posterior}
    p(\vy|\vz,\vx;f) = \mathcal{N} ( \vy ; f(\vz,\vx), \sigma^2\mI),
\end{equation}
where $f:\mathbb{R}^{n+d} \rightarrow \mathbb{R}^{m}$ is a function that maps $\vz$ and $\vx$ to the mean of the distribution, and $\sigma^2$ is a constant scalar that scales the identity covariance matrix.
\end{enumerate}
Now consider a dataset of  $N$ i.i.d samples, $\mathcal{D}=\{(\vx_{i},\vy_{i})\}_{i=1}^N$, generated by the above process. \iffalse, where the corresponding latent variable samples $\{\vz_{i}\}$ are kept hidden and the function $f(\cdot)$ is unknown.\fi Our goal is to estimate the function $f$ within a family of parameterized functions $f_{\boldsymbol\theta}: \mathbb{R}^{n+d} \rightarrow \mathbb{R}^{m}$, e.g. neural networks with weights $\boldsymbol\theta$, by maximizing the log likelihood of the observed data: 
\begin{subequations}\label{eq:max-likelihood}
\begin{align}
    \max_{\boldsymbol\theta}\sum_{i=1}^N\log p(\vy_{i}|\vx_{i};{\boldsymbol\theta}) &= \max_{\boldsymbol\theta}\sum_{i=1}^N \log \int p(\vy_i|\vz, \vx_i)p(\vz)d\vz, \\
    &=\max_{\boldsymbol\theta}\sum_{i=1}^N \log \int \exp\left(-\frac{||f(\vz, \vx_i;{\boldsymbol\theta})-\vy||^2}{2\sigma^2}\right)p(\vz)dz,  
\end{align}
\end{subequations}
In this section, we first introduce the general SOG model which holds for both discrete and continuous  latent variable $\vz$ and solves the optimization problem (\ref{eq:max-likelihood}). We then adapt the SOG model for imitation learning in both the multimodal behavior cloning (BC) and the GAIL settings. We then study the theoretical basis for SOG in the cases of discrete and continuous latent variables.   
\subsection{The General SOG Model}
\vspace*{-.5ex}
%Combining the ideas from \Cref{sec:hard-assignment,sec:continuous}, 

\begin{algorithm}[H]
	\caption{Self-Organizing Generative Model (SOG)}
	\label{alg:sog}
	\begin{algorithmic}[1]
	    \State \textbf{Define}: Loss function $\mathcal{L}\left(\hat{\vy},\vy\right)\coloneqq ||\hat{\vy}-\vy||^2$
		\For {$epoch=1,2,\ldots$}
		     \For {$i=1,2,\ldots$}
		        \State Sample a minibatch of $N_\text{data}$ data points $ (\vx_j,\vy_j)$ from the dataset.
		        \For {$j=1,2,\ldots,N_\text{data}$}
    		        \State Sample $N_z$ latent codes $ \vz_k \sim p(\vz)$. \label{alg:sog:latent-batch}
    		      %  \State Calculate all candidate generated samples $\displaystyle f_\theta(\vz^{k)})$.
    	           \State Calculate $\vz_j\coloneqq\arg\min_{\vz_k}\mathcal{L}\left(f_{\boldsymbol\theta}(\vz_k,\vx_j), \vy_j\right)$.
    	       \EndFor
    	       \State Calculate $ \mathcal{L}_{\mathrm{SOG}}=\sum_{j=1}^{N_\text{data}}\mathcal{L}\left(f_{\boldsymbol\theta}(\vz_j,\vx_j), \vy_j\right)$ and its gradients w.r.t. ${\boldsymbol\theta}$.
    	       \State Update $f_{\boldsymbol\theta}$ by stochastic gradient descent on ${\boldsymbol\theta}$ to minimize $\mathcal L_{\mathrm{SOG}}$.
		    \EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}
We propose \Cref{alg:sog} as a general procedure that applies to both the discrete and continuous latent codes. The main idea of the SOG model is: Given any data pair $(\vx_{i},\vy_{i})$ and the current $f_\theta$, find a $\vz$ such that $\mathcal{L}(\vy_{i} -f_\theta(\vz,\vx_i))$ is minimized; then use this latent code to train the network $f_\theta$. 
 
% \vspace*{-2ex}
\subsection{SOG and SOG-GAIL for Imitation Learning}
\label{sec:sog-imitation}
% \vspace*{-2ex}
To encourage multimodal imitation learning, we introduce two approaches: 
% (1) extending SOG to conditional settings for multimodal BC, and
\begin{enumerate*}[(1)]
    \item Adapting SOG itself for multimodal imitation learning;%, where SOG's latent code is introduced to accommodate multi-modality, and all the state-action pairs in the same trajectory share one latent code.
    \item Combining conditional SOG with GAIL.
\end{enumerate*} We elaborate on each approach in the following.
 
\textbf{Multimodal behavior cloning with SOG.} Inspired by \Cref{alg:sog}, we aim to learn $p_{\boldsymbol\theta}(\va|\vs)$ for multimodal behavior cloning. Enforcing the latent codes to be shared across each trajectory, we obtain \Cref{alg:sog-bc}.

\begin{algorithm}
	\caption{SOG-BC: Multimodal Behavior Cloning with SOG}
	\label{alg:sog-bc}
	\begin{algorithmic}[1]
	    \State \textbf{Define}: Loss function $\mathcal{L}\left(\hat{\va},\va\right)\coloneqq ||\hat{\va}-\va||^2$
	    \State \textbf{Input:} Initial parameters of policy network, $\boldsymbol\theta_0$; expert trajectories $\tau_E\sim\pi_E$
		\For {$i=0,1,2,\ldots$}
    	    \State Sample state-action pairs $\chi_E\sim\tau_E$ with the same batch size.
	        \State Sample $N_z$ latent codes $\displaystyle \vz^{(j)} \sim p(\vz)$ for each trajectory. \label{alg:sog-bc:latent-batch}
            % \State Calculate all candidate generated actions $\displaystyle f_\theta(\vz_{i}, s)$.
            \State Calculate $\vz_E\coloneqq\arg\min_{\vz_j}\hat\E_{\tau_E}\left[\mathcal{L}\left(f_{\boldsymbol\theta}(\vs,\vz_j),    \va\right)\right]$.
            \State Calculate $ \mathcal{L}_{\mathrm{SOG}}=\hat\E_{\tau_E}\left[\mathcal{L}\left(f_{\boldsymbol\theta}(s,\vz_E), \va\right)\right]$ and its gradients w.r.t. $\boldsymbol\theta$.
            \State Update $f_{\boldsymbol\theta}$ by stochastic gradient descent on $\boldsymbol\theta$ to minimize $\mathcal L_{\mathrm{SOG}}$.
		\EndFor
	\end{algorithmic}
\end{algorithm} 

\textbf{Combination of behavior cloning and GAIL with mode separation using SOG.} %
% We propose two approaches and compare them in section \ref{sec:experiments}. The first approach is to directly learn the distribution of possible expert actions over different latent modalities. The other is adding an SOG loss term to GAIL optimization to encourage multi-modality. This loss term also matches policy actions with expert actions at expert states, which is essentially BC. \textbf{Explain your algo }
Motivated by \cite{jena2020augmenting}, in which a weighted combination of the SOG loss and the GAIL surrogate loss is optimized, we introduce Algorithm \ref{alg:sog-gail}. The SOG term encourages multimodal BC, while the GAIL term ensures robustness w.r.t. unseen states via exploration. We evaluate the effectiveness of this model in \Cref{sec:experiments}.

\begin{algorithm}
	\caption{SOG-GAIL}
	\label{alg:sog-gail}
	\begin{algorithmic}[1]
	    \State \textbf{Input:} Initial parameters of policy and discriminator networks, $\boldsymbol\theta_0, \vw_0$; expert trajectories $\tau_E\sim\pi_E$
		\For {$i=0,1,2,\ldots$}
		     \State Sample a batch of latent codes $\vz_i\sim p(\vz)$, and subsequently trajectories $\tau_i\sim\pi_{\boldsymbol\theta_i}(\cdot|\vz_i)$ with the latent code fixed across each trajectory.
		     \State Sample state-action pairs $\chi_i\sim\tau_i$ and $\chi_E\sim\tau_E$ with the same batch size.
		     \State Update the discriminator parameters from $\vw_i$
to $\vw_{i+1}$ with the gradient
            \begin{equation*}
                \mathbb{\hat{E}}_{\tau_i}\left[\nabla_{\vw}\log D_{\vw}(\vs,\va)\right]+\mathbb{\hat{E}}_{\tau_E}\left[\nabla_{\vw}\log \left(1-D_{\vw}(\vs,\va)\right)\right].
            \end{equation*}
            \State Calculate the surrogate loss $\mathcal{L}_\mathrm{PPO}$ using the PPO rule (equation \ref{eq:surrogate})  with the following objective
            \begin{equation*}
                \mathbb{\hat{E}}_{\tau_i}\left[\nabla_{\vw}\log D_{\vw}(\vs,\va)\right]-\lambda_H H(\pi_{\boldsymbol\theta_i}).
            \end{equation*}
            \State Calculate the SOG loss $\mathcal{L}_{\mathrm{SOG}}$ per algorithm \ref{alg:sog-bc}.
            \State Take a policy step from $\boldsymbol\theta_i$ to $\boldsymbol\theta_{i+1}$ w.r.t the objective of $\mathcal{L}_\mathrm{PPO}+\lambda_S \mathcal{L}_{\mathrm{SOG}}$.
		\EndFor
	\end{algorithmic}
\end{algorithm} 
% \vspace*{-2ex}
\subsection{\label{sec:hard-assignment}SOG Analysis: Discrete Latent Variables} 
% \vspace*{-2ex}

We establish a relationship between the SOG and the Expectation-maximization (EM) \cite{dempster1977maximum}, which is a general technique for finding maximum likelihood estimators in latent variable models. In Appendix \ref{appx:em}, we derive the EM algorithm for the maximum likelihood problem of \Cref{eq:max-likelihood}, and obtain an iterative procedure that alternates between the following two steps:
\begin{enumerate}
    \item \textbf{Expectation Step.} At iteration $t$, calculate the posterior probabilities,
    \begin{equation} \label{eq:em-e}
        r_{il}^t= p(\vz_i=l | \{(\vx_i,\vy_i)\}; {\boldsymbol\theta}^{t},\{\pi_j^{t}\}_{j=1}^K).
    \end{equation}
    \item \textbf{Maximization Step.} Update $\boldsymbol\theta^{(t+1)}$ and the prior probabilities $\{\pi_j^{(t+1)}\}_{j= 1}^K$ by maximizing the expectation value,
    \begin{equation} \label{eq:em-m}
        \sum_{k=1}^K \sum_{i=1}^N r_{ik}^t \log p((\vx_i,\vy_i),\vz_i=k \:|\: \boldsymbol\theta,\{\pi_j\}_{j=1}^K).
    \end{equation}
\end{enumerate} 

We provide numerical experiments in \Cref{appx:em} showing that the EM procedure above converges to good local minima. However, the speed of convergence is relatively slow and the storage requirements grow linearly in the number of data points. In addition, we show that the posterior probabilities, $r_{il}^t$'s, asymptotically converge to one-hot assignments. That is, for large enough $t$, $r_{il}^t \rightarrow \gamma_{ik} \in \{0, 1\}$, where for any $i$ there exists a unique $j$ such that $\gamma_{ij} = 1$ and $\gamma_{ik} = 0; \forall k\neq j$. This implies that at convergence, each data point pair $(\vx_{i},\vy_{i})$ is assigned a unique latent code $\vz_{i} = j$. This observation, along with analysis in \Cref{appx:em} supporting the convergence of posterior probabilities to such binary extremes, motivates us to directly search over hard assignments of data points to latent codes. For our numerical experiments, as reported in \Cref{appx:em}, this strategy leads to faster convergence, and achieves better local maxima.  Hence, we can propose the following combinatorial optimization problem  for optimizing the model parameters:
\begin{equation}
\label{eq:gen-cluster}
\begin{aligned}
    \min_{{\gamma}_{ik}} \min_{\boldsymbol\theta} \sum_{k=1}^K \sum_{i=1}^N \gamma_{ik} \norm{f(\vz_{i}=k,\vx_{i};{\boldsymbol\theta}) -\vy_{i}}^2,
\end{aligned}
\end{equation}
where $\gamma_{ik} \in \{0, 1\}$ is a binary indicator variable as defined earlier, and the $L_2$ error follows from the log probabilities in \Cref{eq:em-m}. We shall consider a hard version of the EM algorithm to solve the optimization problem (\ref{eq:gen-cluster}): \begin{enumerate*}[(i)]
    \item For a fixed $\boldsymbol\theta$ greedily pick the best latent code that leads to the least fitting error for each data point. For each data point $i$, this is equivalent to determining the latent code, say $j$,  with  maximum posterior probability, $r_{ij}$, to $1$ and setting the rest of $r_{il}=0$;
    \item Optimize the model parameter $\boldsymbol\theta$ with the corresponding latent code assignments. \iffalse This step makes the additional assumption that the prior is uniform:  $\pi_j=\frac{1}{K}$. \fi
\end{enumerate*}
This hard assignment method is closely analogous to the derivation of the $K$-means algorithm from a corresponding soft EM in Gaussian mixture models \cite{pml1Book}. See \Cref{appx:em} for more details. 

% \vspace*{-2ex}
\subsection{Continuous Latent Variables} \label{sec:continuous}
% \vspace*{-1.5ex}
%\textbf{and the relationship with other non-adversarial generative models.} 
%For the continuous latent variable case, we follow a similar framework as  in the discrete case: (i) For a fixed $\boldsymbol\theta$ search among the samples of continuous latent space for the best code $\vz_i^*$ that leads to the least fitting error for each data point $(\vx_i,\vy_i)$; (ii) Optimize for $\boldsymbol\theta$ by training the model for output $\vy_i$, and input $(\vx_i,\vz_i^*)$.  

The analysis for the continuous case is given in In \Cref{appx:continuous}. Herein, we summarize some of the key characteristics of the continuous case and the resulting SOG algorithm:

\textbf{Relationship with other non-adversarial generative models.} Unlike conventional non-adversarial generative models such as the VAE, the SOG model does not require an encoder.  In VAE, the encoder is used to learn a  posterior distribution $p(\vz| \vx_i,\vy_i;\, \theta)$, whose samples are used to train the decoder. In contrast, SOG trains the decoder by searching for a latent code $\vz$ that maximizes the likelihood $p(\vy | \vx, \vz ;\: \theta)$. By using the basic marginal likelihood identity \cite{chib1995marginal}, one can show that this is equivalent to maximizing the ratio of the posterior to the prior, $\dfrac{p(\vz|\vx_i,\vy_i;\: \boldsymbol\theta)}{p(\vz)}$. In \Cref{appx:continuous}, we %
    % relate the $\max$ operation in SOG to the posterior distribution of the data points and
    show that under reasonable assumptions, the continuous version of the SOG also leads to the maximization of the marginal log-likelihood of the data $p(\mY | \mX;\: \boldsymbol\theta)$. 
    %Related ``encoder-free'' frameworks have been recently considered for image synthesis \cite{bojanowski2017optimizing,hoshen2019non}.
    
    \textbf{Sample complexity.}  For the case of continuous latent variable, the number of  latent code samples required in step \ref{alg:sog:latent-batch} of  \Cref{alg:sog} can grow prohibitively large with the dimensionality of the latent space. However, this dimensionality is a design choice determined by the nature of the dataset. In the scope of imitation learning, which is the focus of this paper (see \Cref{sec:sog-imitation}), low dimensions of the latent code are often sufficient and therefore \Cref{alg:sog-bc} is computationally tractable. Moreover, in \Cref{appx:extended-sog}, we present an extension of \Cref{alg:sog} that is computationally efficient for latent spaces with larger dimensions, and evaluate this extension with visual results.



    % (2) we show that under the assumption of a Gaussian posterior, the likelihood of the data can be expressed exactly in terms of the max operator used in SOG and the mean and variance of the posterior, and (3) Finally, we show that under two different reasonable assumptions the SOG minimizes the log likelihood of the Data.

\textbf{Self-organization and clustering in the latent code space.} In \Cref{appx:lipschitz-bounds} we show analytical results that show how ``self-organization'' might emerge in \Cref{alg:sog}. That is, the latent codes corresponding to nearby data points get organized close to each other. In addition, visual results in \Cref{appx:extended-sog} demonstrate that different regions of the latent space organize towards generating different modes of data. Hence the name of the method is justified.
% \textbf{IMAGE DATA}

%in Further, under the assumption of a uniform prior $p(\vz)$, and by employing the strategy of hard assignment (as used in the derivation of the $K$-means algorithm\cite{pml1Book}) the EM algorithm simplifies to a  case that corresponds to the following objective:
%MLE problem as the following discrete optimization problem, recognizing that the log of the assumed Gaussian likelihood is directly translated to $\normltwo$ norm:
%\begin{equation}
%\label{eq:gen-cluster}
%\begin{aligned}
 %   \min_{{l}_{ik}} \min_\theta %\sum_{k=1}^K \sum_{i=1}^N %l_{ik} \norm{f(\vz_{i}=k,\vx_{%i};\theta) -\vy_{i}}^2,
%\end{aligned}
%\end{equation}
%where $l_{ik} \in \{0, 1\}$ is a binary indicator variable, and for any $i$ there exists one and only one $j$ such that $l_{ij} = 1$ while $l_{ik} = 0$ for $k\neq j$. This implies that the data point pair $(\vx_{i},\vy_{i})$ is assigned the latent code $\vz_{i} = j$ %
%(equivalently, $\vz_{i} = e_j$, the corresponding one-hot code)
%and the function  $f_\theta(\vz_{i}=j,\vx_{i})$ is used to estimate $\vy_{i}$. 

%Let $\mathcal{C}_k = \{i \given l_{ik} = 1\}$ be the set of all data point indices that are assigned to the latent code $k$. Then solving the optimization problem in \cref{eq:gen-cluster} corresponds to determining an optimal clustering of the data points into $K$ sets, $\{\mathcal{C}_{1}, \cdots, \mathcal{C}_K\}$, such that the log-likelihood of the data is maximized by the respective generators $f_{\theta}^{(k)}(\cdot) \equiv f_\theta(\vz_{i}=k, \cdot)$, for $k=1, \cdots, K$.
% One pair of data, $(\vx_{i}, \vy_{i})$, defines a single-point mapping function $m_i: m_i(\vx_{i}) = \vy_{i}$. % This functional view of the data-label pairs is illuminating. It helps to recognize that a distance metric among the mapping functions (including $f^{(k)}_\theta$) can be induced from a metric in the data (label?) space
%Therefore \cref{eq:gen-cluster} can be re-written as
%\begin{align}
%\label{eq:cluster-opt}
 %   &\min_{\{\mathcal{C}_1,\cdo%ts,\mathcal{C}_K\}} \; %\sum_{k=1}^K \;\; %\left(\min_{f^{(k)}} \; %\sum_{(\vx, \vy) \in %\mathcal{C}_k} \norm{\vy - %f^{(k)}(\vx)} \right)
    % \\ =& %\min_{\{\mathcal{C}_1,\cdot%s,\mathcal{C}_K\}} \; %\sum_{k=1}^K \;\; \left( %\min_\theta \; \sum_{i \in %\mathcal{C}_k} \xi(f^{(k)}, %(\vx_i, \vy_i)) \right)
%\end{align}

%Again we compare \cref{eq:cluster-opt} with the objective of $K$-means clustering algorithm in \cref{prob:kmeans} to emphasize their similarity. This reveals that the case of discrete latent codes can be viewed as a generative clustering problem, where one jointly optimizes for both cluster assignments of data points and  the functions $\{f^{(k)}\}_{k=1}^K$ to fit the data points within each cluster.

%\begin{align}
%\label{prob:kmeans}
%    \min_{\{\mathcal{C}_1,\cdot%s,\mathcal{C}_K\}} \; %\sum_{k=1}^K \;\; %\left(\min_{\mu_k} \; %\sum_{\vx_{i} \in %\mathcal{C}_k} \norm{\vx_{i} - %\mu_k} \right)
    % = \min_{\{\mathcal{C}_1,\c%dots,\mathcal{C}_K\}} \; %\sum_{k=1}^K \;\; \left( %\min_{\{\mu_1,\cdots,\mu_K\%}} \; \sum_{\vx_{i} \in %\mathcal{C}_k} %\xi{(\vx_{i}, \mu_k)} %\right)
%\end{align}

%Note that the $f^{(k)}$ in \cref{eq:cluster-opt} are assumed to share the parameter $\theta$ and differ only due to the fed-in latent codes. This assumed form of $f^{(k)}$ can be considered as a regularization that prevents the learning of multiple completely disjoint models (one for each latent code assignment $\vz=k$) and in practice boosts the training process, because $\theta$ receives feedback from all data points regardless of the modality.

% This analogy to $K$-means is important because we can take $K$-means' approach to address this problem, which is the EM algorithm or its hard-assignment version. We show in the appendix that algo that solves this problems can be derived from the EM framework, and $K$-means' approach leads to SOG.

% Thus, the case of discrete latent codes can be viewed as a Generative Functional Clustering Problem (GFCP), where one jointly optimizes for both cluster assignments of data points and  the parameters $\theta$ that construct the functions $f_\theta(\cdot, \cdot)$.

% If $f_\theta(\cdot, \cdot)$ is realized using a DNN with a large enough number of parameters then one can achieve a small enough reconstruction error for almost any clustering of the input data. These clusters, however, need not correspond to the naturally occurring distinct modes present in  expert demonstrations: in principle, a DNN can learn any function, however non-smooth, given enough parameters, training data and computing power.

%The problem in \cref{eq:gen-cluster} (or \cref{eq:cluster-opt}) is a combinatorial optimization problem and a number of algorithms can potentially be used to find good minima. There are, however, several challenges of which perhaps the most important one relates to the approximation capabilities of DNNs. If $f_\theta(\cdot, \cdot)$ is realized using a DNN with a large enough number of parameters then one can achieve a small enough reconstruction error for almost any clustering of the input data. These clusters, however, need not correspond to the naturally occurring distinct modes present in  expert demonstrations: in principle, a DNN can learn any function, however non-smooth, given enough parameters, training data and computing power. To avoid such complex mapping in the decoder, we adopt the iterative framework of expectation-maximization (EM). The underlying goal is to perform least squares regression between $\vx$, $\vy$ pairs (conditioned on the one-hot latent codes) in incremental steps, while ensuring smoothness of the function $f_\theta$ w.r.t. its arguments. As shown in \Cref{lipschitz-bounds} our iterative EM framework ensures that data pairs $(\vx,\vy)$ that are close to each other, and hence, could be considered as belonging to the same mode, are mapped to the same latent variable $\vz$. Thus, data points that are close to each other  use the same mapping $f_\theta(\vz,\cdot)$, keeping it smooth and less complex.

%The connection between the case of discrete latent code and the $K$-means algorithm motivates the following iterative  optimization paradigm that we have termed as the SOG:
%\begin{enumerate*}[(a)]
 %   \item For a fixed $\theta$ greedily pick the best latent code that leads to the least fitting error for each data point;
 %   \item Optimize the model parameter $\theta$ assuming the picked latent code. Repeat.
%\end{enumerate*}





% The likelihood of an individual datapoint $\vy$ can be written as:
% \begin{subequations} \label{eq:likelhood}
%     \begin{align}
%     \displaystyle 
%     p_\theta(\vy)   & = \E_{\vz\sim p(\vz)} \left[ p_\theta(\vy | \vz)\right] \label{subeq:likelihood} \\
%                     & = \E_\ensemble \left[\frac{1}{N_z}\sum_{i=1}^{N_z} p_\theta(\vy | \vz_{i})\right], \hspace{0.45in} \vz^{(1)},\ldots, \vz^{(N_z)} \stackrel{\mathrm{i.i.d}}{\sim} p(\vz) \label{subeq:montecarlo1}
%     \end{align}
% \end{subequations}
% where in \ref{subeq:montecarlo1} the variable under expectation is replaced with its empirical mean. Taking the logarithm of both sides we obtain:
% \begin{subequations} \label{eq:log-likelihood}
%     \begin{align}
%     \displaystyle 
%     \log p_\theta(\vy) & = \log\E_\ensemble \left[\frac{1}{N_z}\sum_{i=1}^{N_z} p_\theta(\vy | \vz_{i})\right] \\
%         & = \log\E_\ensemble \left[C \sum_{i=1}^{N_z}  \frac{1}{N_z}\exp\left(-\frac{||f_\theta(\vz_{i})-\vy||^2}{2\sigma^2}\right)\right] \label{subeq:montecarlo2} \\
%         & \geq \E_\ensemble \left[ \log \left( C \sum_{i=1}^{N_z} \frac{1}{N_z}\exp\left(-\frac{||f_\theta(\vz_{i})-\vy||^2}{2\sigma^2}\right) \right)\right] \label{subeq:jensen}  \\
%         & \geq \E_\ensemble \left[\log \left( C\max_{i} \left\{ \frac{1}{N_z} \exp\left(-\frac{||f_\theta(\vz_{i})-\vy||^2}{2\sigma^2}\right)\right\}\right)\right] \label{subeq:boeltzmann} \\
%         & = C' -\frac{1}{2\sigma^2} \E_\ensemble \left[ \min_{i}||f_\theta(\vz_{i})-\vy||^2\right]. \label{subeq:simplified-min}
%     \end{align}
% \end{subequations}
% Equation \ref{subeq:montecarlo2} is the density of the Gaussian distribution in equation \ref{eq:posterior}, with constants $C$ (and $C'$) defined as appropriate. Inequality \ref{subeq:jensen} follows from Jensen's inequality, and is shown in Appendix \ref{appx:proof} to provide a tight bound for large enough $N_z$. Moreover, (\ref{subeq:boeltzmann}) is obtained by keeping only the largest summand. This bound also gets tighter as $\sigma$ decreases. As apparent from (\ref{subeq:simplified-min}), $\sigma$ only plays a role in scaling the magnitude of the gradient. 

% We optimize the lower bound of the maximum likelihood objective, by taking gradient of (\ref{subeq:simplified-min}). We also approximate the expectation in (\ref{subeq:simplified-min}) with one sample. Altogether, we first draw $N$ i.i.d samples $\displaystyle \vz_{i}$, then up to a constant factor the gradient of the log-likelihood can be written as:
% \begin{equation}
%     \displaystyle 
%     \nabla_\theta \log p_\theta(\vy)  \approx -\nabla_\theta \min_i
%     ||f_\theta(\vz_{i})-\vy||^2
% \end{equation}
% \vspace*{-2ex}

